Large Language Models Are Zero-Shot Text Classifiers

Retrained large language models (LLMs) have become extensively used across various sub-disciplines of natural language processing (NLP). In NLP, text classification problems have garnered considerable focus, but still faced with some limitations related to expensive computational cost, time consumption, and robust performance to unseen classes. With the proposal of chain of thought prompting (CoT), LLMs can be implemented using zero-shot learning (ZSL) with the step by step reasoning prompts, instead of conventional question and answer formats. The zero-shot LLMs in the text classification problems can alleviate these limitations by directly utilizing pretrained models to predict both seen and unseen classes. Our research primarily validates the capability of GPT models in text classification. We focus on effectively utilizing prompt strategies to various text classification scenarios. Besides, we compare the performance of zero shot LLMs with other state of the art text classification methods, including traditional machine learning methods, deep learning methods, and ZSL methods. Experimental results demonstrate that the performance of LLMs underscores their effectiveness as zero-shot text classifiers in three of the four datasets analyzed. The proficiency is especially advantageous for small businesses or teams that may not have extensive knowledge in text classification.

==> backup.tex <==
% \begin{table*}[h!]
% \centering
% \caption{\small{dataset}}
% \begin{tabular}{lccc|cccc}
% \toprule
% & \multicolumn{3}{c}{Tweets} & \multicolumn{4}{c}{Ecommerce} \\
% \cmidrule(r){2-4} \cmidrule(r){5-8}
% & Positive & Neural & Negtive & Household & Clothing \& Accessories & Books & Electronics \\
% \midrule
% Train          & 18046   & 7713 & 15398 & 9656  & 4335 & 5910 & 5310 \\
% Test           & 41   & 16 & 43 & 38  & 17 & 24 & 21 \\
% \bottomrule
% \end{tabular}
% \end{table*}


% experiment results
% https://github.com/lorrespz/NLP-text-analysis

% "Coronavirus tweets NLP - Text Classification"
% code: https://www.kaggle.com/code/lorresprz/covid19-tweet-analysis-rnn-lstm-others

% Ecommerce Text Classification
% https://www.kaggle.com/datasets/saurabhshahane/ecommerce-text-classification

% Financial Sentiment Analysis
% https://www.kaggle.com/datasets/sbhatti/financial-sentiment-analysis

% SMS Spam Collection Dataset
% https://www.kaggle.com/datasets/uciml/sms-spam-collection-dataset

% \begin{table}[h!]
% \centering
% \caption{\small{Results}}
% \begin{tabular}{lccc|ccc}
% \toprule
% & \multicolumn{3}{c}{Tweets} & \multicolumn{3}{c}{Ecommerce} \\
% \cmidrule(r){2-4} \cmidrule(r){5-7}
% & ACC & F1 & AUC & ACC & F1 & AUC \\
% \midrule
% MNB          & 0.44   & 0.4329 & 0.6035 & 0.23  & 0.2178 & 0.5048 \\
% LG           & 0.42   & 0.3028 & 0.5561 & 0.41  & 0.2959 & 0.6643 \\
% RF           & 0.45   & 0.3598 & 0.6402 & 0.49  & 0.3858 & 0.6632 \\
% DTC          & 0.45   & 0.3978 & 0.5477 & 0.44  & 0.4212 & 0.6063 \\
% KNN          & 0.34   & 0.2581 & 0.5210 & 0.44  & 0.3973 & 0.6277 \\
% RNN          & 0.8    & 0.7988 & 0.9301 & 0.96  & 0.9612 & 0.9958 \\
% LSTM         & 0.83   & 0.8000 & 0.9260 & 0.95  & 0.9529 & 0.9866 \\
% GRU          & 0.8    & 0.8036 & 0.9212 & 0.93  & 0.9345 & 0.9956 \\
% Llama2-70B  & 0.54   & 0.5037 & -      & 0.90  & 0.7295 & - \\
% GPT3.5       & 0.54   & 0.4787 & -      & 0.88  & 0.8835 & - \\
% GPT4         & 0.57   & 0.5572 & -      & 0.96  & 0.9605 & - \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}[h!]
% \centering
% \caption{\small{Results}}
% \begin{tabular}{lccc|ccc}
% \toprule
% & \multicolumn{3}{c}{Tweets} & \multicolumn{3}{c}{Ecommerce} \\
% \cmidrule(r){2-4} \cmidrule(r){5-7}
% & ACC & F1 & AUC & ACC & F1 & AUC \\
% \midrule
% MNB          & 0.3933 & 0.3639 & 0.5531 & 0.2667 & 0.2546 & 0.5289 \\
% LG           & 0.4333 & 0.3488 & 0.5404 & 0.3867 & 0.2820 & 0.6529 \\
% RF           & 0.4467 & 0.3184 & 0.6184 & 0.5133 & 0.4410 & 0.7267 \\
% DTC          & 0.4733 & 0.4105 & 0.5602 & 0.5467 & 0.5412 & 0.6964 \\
% KNN          & 0.3800 & 0.3486 & 0.5216 & 0.3600 & 0.3159 & 0.5891 \\
% RNN          & 0.7400 & 0.7186 & 0.8925 & 0.9600 & 0.9598 & 0.9964 \\
% LSTM         & 0.7867 & 0.7619 & 0.8925 & 0.9467 & 0.9468 & 0.9854 \\
% GRU          & 0.8200 & 0.8106 & 0.9226 & 0.9400 & 0.9401 & 0.9883 \\
% \hline
% Llama2-70B   & 0.5200 & 0.3523 & -      & 0.8067 & 0.6644 & - \\
% GPT-3.5      & 0.5333 & 0.4943 & -      & 0.8867 & 0.8935 & - \\
% GPT-4        & 0.5267 & 0.5095 & -      & 0.9000 & 0.9078 & - \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}[h!]
% \centering
% \caption{\small{Results}}
% \begin{tabular}{lccc|ccc}
% \toprule
% & \multicolumn{3}{c}{Financial Sentence} & \multicolumn{3}{c}{SMS} \\
% \cmidrule(r){2-4} \cmidrule(r){5-7}
% & ACC & F1 & AUC & ACC & F1 & AUC \\
% \midrule
% MNB          & 0.39   & 0.2929 & 0.5306 & 0.81  & 0.7085 & 0.8254 \\
% LG           & 0.52   & 0.3073 & 0.6143 & 0.84  & 0.5116 & 0.5155 \\
% RF           & 0.55   & 0.3849 & 0.5994 & 0.90  & 0.6947 & 0.6481 \\
% DTC          & 0.44   & 0.3665 & 0.5249 & 0.85  & 0.6315 & 0.6194 \\
% KNN          & 0.49   & 0.3894 & 0.5652 & 0.85  & 0.6315 & 0.6194 \\
% RNN          & 0.51   & 0.4451 & 0.6465 & 0.97  & 0.9263 & 0.8846 \\
% LSTM         & 0.63   & 0.5088 & 0.7048 & 0.99  & 0.9786 & 0.9943 \\
% GRU          & 0.63   & 0.5520 & 0.7336 & 0.99  & 0.9771 & 0.9615 \\
% Llama2-70B   & 0.71   & 0.7062 & -      & 0.75  & 0.4521 & - \\
% GPT3.5       & 0.65   & 0.6538 & -      & 0.97  & 0.9395 & - \\
% GPT4         & 0.70   & 0.6933 & -      & 0.99  & 0.9786 & - \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}[h!]
% \centering
% \caption{\small{Results}}
% \begin{tabular}{lccc|ccc}
% \toprule
% & \multicolumn{3}{c}{Financial Sentence} & \multicolumn{3}{c}{SMS} \\
% \cmidrule(r){2-4} \cmidrule(r){5-7}
% & ACC & F1 & AUC & ACC & F1 & AUC \\
% \midrule
% MNB          & 0.4533 & 0.3632 & 0.5563 & 0.7600 & 0.6425 & 0.7346 \\
% LG           & 0.5200 & 0.3066 & 0.5427 & 0.8333 & 0.4545 & 0.4808 \\
% RF           & 0.5133 & 0.3453 & 0.5990 & 0.9067 & 0.7678 & 0.7346 \\
% DTC          & 0.4067 & 0.3446 & 0.5060 & 0.8667 & 0.7337 & 0.7538 \\
% KNN          & 0.4800 & 0.3620 & 0.5614 & 0.8400 & 0.6384 & 0.6327 \\
% RNN          & 0.6333 & 0.5797 & 0.7874 & 0.9800 & 0.9558 & 0.9462 \\
% LSTM         & 0.6533 & 0.4627 & 0.7293 & 0.9600 & 0.9005 & 0.8500 \\
% GRU          & 0.6933 & 0.5767 & 0.7928 & 0.9867 & 0.9699 & 0.9500 \\
% \hline
% Llama2-70B   & 0.7000 & 0.5230 & -      & 0.7267 & 0.4441 & - \\
% GPT-3.5      & 0.6667 & 0.6683 & -      & 0.8733 & 0.7996 & - \\
% GPT-4        & 0.7133 & 0.7096 & -      & 0.9733 & 0.9467 & - \\
% \bottomrule
% \end{tabular}
% \end{table}

